Modeling Shared Responses in Neuroimaging Studies through MultiView ICA

Group studies involving large cohorts of subjects are important to draw general conclusions about brain functional organization. However, the aggregation of data coming from multiple subjects is challenging, since it requires accounting for large variability in anatomy, functional topography and stimulus response across individuals. Data modeling is especially hard for ecologically relevant conditions such as movie watching, where the experimental setup does not imply well-defined cognitive operations. We propose a novel MultiView Independent Component Analysis (ICA) model for group studies, where data from each subject are modeled as a linear combination of shared independent sources plus noise. Contrary to most group-ICA procedures, the likelihood of the model is available in closed form. We develop an alternate quasi-Newton method for maximizing the likelihood, which is robust and converges quickly. We demonstrate the usefulness of our approach first on fMRI data, where our model demonstrates improved sensitivity in identifying common sources among subjects. Moreover, the sources recovered by our model exhibit lower between-session variability than other methods.On magnetoencephalography (MEG) data, our method yields more accurate source localization on phantom data. Applied on 200 subjects from the Cam-CAN dataset it reveals a clear sequence of evoked activity in sensor and source space. The code is freely available at https://github.com/hugorichard/multiviewica.

==> sec/sharedresponsemod.tex <==
%!TEX root = ../main.tex

For a group study in neuroimaging, the data can be represented as a collection of matrices $\{X_i\in \mathbb{R}^{v \times d}\}_{i=1}^m$, where $v$ is the number of voxels, $d$ is the number of time repetitions and $m$ is the number of subjects.
The Shared Response Model~\cite{chen2015reduced} provides an efficient way to perform dimensionality reduction for data with these characteristics.

The model is motivated by defining a likelihood related to the one for probabilistic Canonical Correlation Analysis~\cite{bach2005probabilistic}. In SRM, the data pertaining to each subject is modelled as the projection into individual anatomy of a shared response $S\in \mathbb{R}^{k \times d}$; that is,

\begin{equation}
    X_i = W_iS + E_i\,. \label{eq:srm1}
\end{equation}

The original Shared Response Modeling (SRM) paper~\cite{chen2015reduced} suggests that the bases $W_i$ should be thought of as representing the individual functional topographies, and $S$ is a shared matrix of feature responses. The model in equation~\ref{eq:srm1} also includes an additive error term $E_i$, suited to model the experimental noise.

In order to make the optimization of the likelihood for the above model efficient, the bases $W_i$ are assumed to be orthogonal. This is a limitation to the expressiveness of the model. In appendix~\ref{sec:app_identifiability}, we show that this assumption impinges on the identifiability of the model.

% Our proposed Multiview ICA method obviates this problem by proposing a procedure with identifiability guarantees coming from the Independent Component Analysis theory, as we describe in section~\ref{sec:mvica}. 
